M dwarf spectral indices at moderate resolution: accurate $T_{\mathrm{eff}}$ and [Fe/H] for 178 southern stars

We present a spectroscopic and photometric calibration to derive effective temperatures $T_{\mathrm{eff}}$ and metallicities [Fe/H] for M dwarfs, based on a Principal Component Analysis of 147 spectral indices measured off moderate resolution $R \sim 11\,000$), high S/N ($>100$) spectra in the $\lambda \lambda$ 8390-8834 region, plus the J$-$H color. Internal uncertainties, estimated by the residuals, are 81 K and 0.12 dex, respectively, for $T_{\mathrm{eff}}$ and [Fe/H], the calibrations being valid for 3050 K $< T_{\mathrm{eff}} <$ 4100 K and $-$0.45 $<$ [Fe/H] $<$ $+$0.50 dex. The PCA calibration is a competitive model-independent method to derive $T_{\mathrm{eff}}$ and [Fe/H] for large samples of M dwarfs, well suited to the available database of far-red spectra. The median uncertainties are 105 K and 0.23 dex for $T_{\mathrm{eff}}$ and [Fe/H], respectively, estimated by Monte Carlo simulations. We compare our values to other works based on photometric and spectroscopic techniques and find median differences 75 $\pm$ 273 K and 0.02 $\pm$ 0.31 dex for $T_{\mathrm{eff}}$ and [Fe/H], respectively, achieving good accuracy but relatively low precision. We find considerable disagreement in the literature between atmospheric parameters for stars in common. We use the new calibration to derive $T_{\mathrm{eff}}$ and [Fe/H] for 178 K7-M5 dwarfs, many previously unstudied. Our metallicity distribution function for nearby M dwarfs peaks at [Fe/H]$\sim$-0.10 dex, in good agreement with the RAVE distribution for GK dwarfs. We present radial velocities (internal precision 1.4 km/s) for 99 objects without previous measurements. The kinematics of the sample shows it to be fully dominated by thin/thick disk stars, excepting the well-known high-velocity Kapteyn's star.

==> References.tex <==
M DWARF METALLICITIES AND GIANT PLANET OCCURRENCE:
IRONING OUT UNCERTAINTIES AND SYSTEMATICS
\url{https://iopscience.iop.org/article/10.1088/0004-637X/791/1/54/pdf}

Trumpeting M dwarfs with CONCH-SHELL: a catalogue of nearby cool host-stars for habitable exoplanets and life
\url{https://watermark.silverchair.com/stu1313.pdf?token=AQECAHi208BE49Ooan9kkhW_Ercy7Dm3ZL_9Cf3qfKAc485ysgAAAqwwggKoBgkqhkiG9w0BBwagggKZMIIClQIBADCCAo4GCSqGSIb3DQEHATAeBglghkgBZQMEAS4wEQQMy52MPq6DEs4ZWuVvAgEQgIICXxunS_pC0Avyi2Aw_kbR5moj-lcHKRwIUcFjPDMMSzi-iukZ465-cbO_B48hv7rD5Mv-IPM0FbBRG4AUOcuYvTgsmYFzVvOuTRPDgIh9ocJxUw0dLDnLOtwAVI0QUQ27BUNS27Bwhg8M3MfMV7zy9Tosl213lKWdwHPydCGiZgrLRPbyH9IQEFqA98QTD-DvTJn51wqbE1i1nZuD9EojGfg9hhUQGt92pC7m654a2x0Lofgj3c7FRixptpjNQKS02iXdDBpJUEMc4YphGdOqM3jdkp4vn9bLgquhHjzelTmwMp5PpiGvmR5TEA0E_Tqm_TXGDfBWNIPs45YiLQCiiFn3lPVHIE0O1PD9pP7WlATQ2WwnBXYnA-XD6X1vRJwXv6LZvd0akAjBTiB2MiAV_Ond8ELX8r7Sd-DB2IZPoamMkk7J02V-kK8qaPQV2h8Y-sTqIbbk73Xo9Skf3AEwZaMhuB6VzkzreplwuSPrKMSXLKKHB3cadg5_QtqjGd9daFZwzPNZAi2ZOoGoz0jA64XeuRfqKWTygW_wQlk3UHDxOwu_zOVWiphLurnUNEN_-ahpztu1I804jsWN2gEbUy5iUe3KMbZz9QOR3RpgJLzGUR6BfwcKREvSFVMNlCq9VUmtaGui8vPqlGTXuBgZ88iXQPX2h3N8vXsG9s2_yTAogDnZ96vonogI1NSp7KtZ8neDU783xb9Ki6saViZQ7LpuU55wdy5C1cNkc3iJnqD1W9CMwD3ApiQExX7_wX0zhfmHT53xFEr-sWLcxkgGNuBZK6SlU3njgWKrAP--z8Q}

A PCA approach to stellar effective temperatures
\url{https://ui.adsabs.harvard.edu/#abs/2013A\%26A...553A..95M}
